An MCMC sampling of densest $k$-sub-graphs of regular graphs with connected complement graph

We present an exclusion process based approach for sampling densest $k$-sub-graphs from regular graphs $L$ with connected complement. By interpreting an exclusion process as a Markov chain on a corresponding Token Graph $\mathfrak{L}_k$, we make use of classical Markov chain theory to obtain quantitative bounds on the convergence speed depending on the geometry of $L$, which are sharp in the sens that variations in the valency lead to an equality, which is $1$, for the geometric bounds in the case of a complete graph. We propose an algorithm which makes use of this particle view to avoid excessive memory use due to the state space size and discuss the regularity and connectivity condition on $L$ and $L^c$ in the Outlook.

==> chapters_adjusted/montecarlo.tex <==
\textbf{Outline of this section:} Particle systems on finite graphs represent in a canonical form vertex-induced sub-graphs. This section is dedicated to the discussion of a generalized exclusion process which converges to a stationary distribution which assigns to any particle configuration a weight which is inversely proportional to its density, defined by its edge density as an induced sub-graph. We complete the chapter by proposing an algorithmic approach to sampling densest sub-graphs from regular graphs using MCMC techniques with an underlying Markov chain induced by a generalized exclusion process. We quantify its convergence speed in terms of the geometrical properties of the associated kPG and give an explicit form of the stationary distribution. 
